Neural Architecture Search Over a Graph Search Space

Neural Architecture Search (NAS) enabled the discovery of state-of-the-art architectures in many domains. However, the success of NAS depends on the definition of the search space. Current search spaces are defined as a static sequence of decisions and a set of available actions for each decision. Each possible sequence of actions defines an architecture. We propose a more expressive class of search space: directed graphs. In our formalism, each decision is a vertex and each action is an edge. This allows us to model iterative and branching architecture design decisions. We demonstrate in simulation, and on image classification experiments, basic iterative and branching search structures, and show that the graph representation improves sample efficiency.

==> Graph Nips19/abstract.tex <==
\begin{abstract}
Neural Architecture Search (NAS) enabled the discovery of state-of-the-art architectures in many domains.
However, the success of NAS depends on the definition of the search space. 
Current search spaces are defined as a static sequence of decisions and a set of available actions for each decision.
Each possible sequence of actions defines an architecture.
We propose a more expressive class of search space: directed graphs.
In our formalism, each decision is a vertex and each action is an edge.
This allows us to model iterative and branching architecture design decisions.
We demonstrate in simulation, and on image classification experiments, basic iterative and branching search structures, and show that the graph representation improves sample efficiency.
\end{abstract}

%We also propose a novel architecture for a neural agent that is capable to learn to explore graph search spaces.

==> Graph Nips19/acknowledgements.tex <==
\section{Acknowledgements}
We would like to thank
Tomas Effenberger,
David Dohan,
Damien Vincent,
Sylvain Gelly,
Noe Lutz,
Vijay Vasudevan,
Quoc Le and the whole
Google AI team in Zurich for influencing and contributing to the ideas and results presented in this paper.

==> Graph Nips19/conclusions.tex <==
\section{Conclusion}

We introduced a more expressive formalism for defining neural architecture search spaces, and a novel dynamic controller that is able to efficiently learn to explore this new class of search spaces.
Our experiments show significant improvements in sample efficiency in exploring common iterative or branching architecture design patterns.
As next steps, we plan to apply this method to other neural architecture search tasks and design a new class of search spaces that are not feasible in the linear form.

==> Graph Nips19/experiments.tex <==
\section{Experiments}

% INTRO
We demonstrate the potential benefit of performing architecture search with a graph search space, and the ability of the dynamic controller to optimize this space, using two artificial tasks.
We present hand-crafted optimization problems that are representative of the branching and iterative components of architecture design.
For each toy task, we compare the efficacy of modeling the search space as a sequence or a graph.

% TASKS OVERVIEW
The first task models the iterative process of stacking layers.
The second task models a decision that involves branching, such as picking the optimizer among few alternatives, and tuning its parameters.
In both tasks we demonstrate that expressing the search space as a graph significantly improves the sample efficiency of the controller.

% EXPERIMENTS SHARED SETUP
% Not true, so commented out
% In all experiments we use the dynamic neural controller introduced in Section~\ref{sec:arch}, trained with the REINFORCE algorithm~\citep{williams1992simple}./
% All experiments are repeated $4$ times, and the results are averaged.

\subsection{Stack layers toy task}


\begin{wrapfigure}{r}{0.5\textwidth}
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/addlayer.pdf}
\caption{Results for the ``stack layers'' task. Best reward over time averaged across 10 replicas. The shaded area corresponds to maximum and minimum reward achieved by the replicas. %The task is solved by achieving reward $1$.
}
\label{fig:addlayers_results}
\end{center}
\end{wrapfigure}





% \begin{figure}
% \centering
% \begin{minipage}{.5\textwidth}
% \centering
% \includegraphics[width=1.0\linewidth]{figures/architecture.pdf}
% \caption{
% Architecture for one timestep of the dynamic RNN controller. Inputs are highlighted in green, outputs in blue. The timestep independent network is highlighted in red, the timestep dependent network in yellow.
% \label{fig:architecture}
% }
% \end{minipage}%
% \begin{minipage}{.5\textwidth}
% \centering
% \includegraphics[width=0.5\linewidth]{figures/nn_addlayer_graph.pdf}
% \caption{Graph search space used in the Cifar10 experiments. The controller can terminate at any moment. Additionally, conditional decisions are possible within each layer.}
% \label{fig:nn_search_space}
% \end{minipage}
% \end{figure}

% DESCRIPTION OF THE TASK
The first task is based on an iterative, or cyclic, search space.
This task simulates the process of constructing a neural network with a variable number of layers.
%In this task, a search space over a simulated ``number of layers'', $n$ is defined.
The controller must choose the optimal number of layers $n$.
% REWARD
The reward in this simulation is defined as $-(n - L)^2$.
The maximum reward is achieved by constructing a network with exactly $L$ layers.
Otherwise, a squared error penalty is applied.
%Note that extensions of this tasks might include setting different parameters for each layer, such as number of units or learning rate.

% DESCRIPTION OF HOW THE TASK IS REPRESENTED WITH THE SEARCH SPACES
To compare the two approaches, we define both linear and graph instances of this search space.
% Both are shown in Figure~\ref{fig:addlayers_vis}.
% LINEAR
A linear search space describing this task is defined as a sequence of states of length $2L$.
At each state only 2 actions are available, either to add 1 extra layer or to terminate.
% GRAPH
The graph search space is defined as a single state with 2 actions.
The action to add a new layer is represented as a cyclic edge on the unique state.
The second action transitions to the terminal state, after which no more layers are added. %We designed such iterative search spaces as more complex tasks might involve setting different parameters for each layer (e.g: number of units).

% EXPERIMENT HPARAMS
For the following experiments, $L$ is set to $10$.
The reward is normalized to $[0,1]$ range. We use REINFORCE to optimize controller,
with learning rate 0.001 and entropy regularization 0.1.


% RESULTS DISCUSSION
The results are summarized in Figure~\ref{fig:addlayers_results}.
The graph search space improves training speed, converging to the maximum reward much more rapidly.
In fact, in this search space, linear fails to attain maximal reward in the number of trials ran, 200. In the linear case the controller is forced to output a fixed number of decisions, which, in this task, forces an arbitrary upper bound (for we chose $2L$ based on prior knowledge of the simulated task).
However, the graph search space has no bound on number of iterations,
thus, lifting the constraint on the maximum number of layers required by the linear version.
The graph search space could be harder to optimize, because it may accept an infinite number of trajectories.
However, despite the added complexity, the dynamic controller is able to solve the task more effectively searching over the graph. % Finally, note that while sharing states is possible using a linear search space (and was done in~\citep{zoph2017b}), the key advantage of graph based search space is that it allows to model efficiently deciding on the number of layers.

% Again, not sure we need this visualization
% \begin{figure}[t]
% \centering
% \subfigure[Search space as a sequence]{\includegraphics[width=0.6\linewidth]{figures/addlayer_lin.pdf}}
% \subfigure[Search space as a graph]{\includegraphics[width=0.25\linewidth]{figures/addlayer_fs.pdf}}
% \caption{``Stack layers'' task of length $L$. The controller is maximally rewarded if it makes $L$ consecutive steps and is penalized for taking more or fewer steps. This is inspired by the common phenomenon in constructing architectures where using either too few, or too many layers leads to poorer performance.}
% \label{fig:addlayers_vis}
% \end{figure}



\subsection{Select an optimizer toy task}

% NOTE: THE STRUCTURE OF THIS SUBSECTION MIRRORS THE ONE OF THE FIRST TOY TASK.

\begin{figure}[t]
\centering
\subfigure[Search space as a sequence]{\includegraphics[width=0.48\linewidth]{figures/new_branch_lin.pdf}}
\subfigure[Search space as a graph]{\includegraphics[width=0.48\linewidth]{figures/new_branch_fsm.pdf}}
\caption{``Select an optimizer'' toy task with $B$ branches.}
\label{fig:branch_vis}
\end{figure}

\begin{figure}[t]
\begin{center}
\subfigure[Results for two branches environment.]{\includegraphics[width=0.49\linewidth]{figures/max_two_branch_eps0_1.pdf}}
\subfigure[Results for four branches environment.]{\includegraphics[width=0.49\linewidth]{figures/max_four_branch_eps0_1.pdf}}
\caption{Results for the ``select an optimizer'' task. Best reward over time averaged across 10 replicas for two branch (left) and four branch (right) versions of the environment. The shaded area corresponds to maximum and minimum reward achieved by the replicas.
%The task is solved by achieving reward $1$.
}
\label{fig:branch_results}
\end{center}
\end{figure}

% DESCRIPTION OF THE TASK
The second task is based on an branching choices search space.
This task simulates picking between several optimizers, then choosing optimizer specific hyper-parameters, such as learning rate or decay rate.
Thus, we designed a toy task that requires the controller to first choose an optimizer $b$ among $B$ options, and then chooses 4 optimizer specific hyper-parameters: $p_1,p_2,p_3,p_4$.
For the following experiments $B$ may take a value in $\{2, 4\}$, and each of the hyperparameter can be set to a value in the range $[1, 100]$.




% REWARD
The reward is defined as follows. The agent is maximally rewarded for setting all the 4 relevant hyperparameters to the value of $50$.
Let  $M(b,p_1,p_2,p_3,p_4)=\argmin_{i=1,\ldots,4} p_i \neq 50$, i.e. $M$ denotes index of the first \emph{incorrect} $p_i$. Then, the unnormalized reward is defined as: $r = -(p_M - 50)^2 - \sum_{i=M+1}^4 50^2$.
%$$r(b,p_1,p_2,p_3,p_4)=-(p_M - 50)^2 - \sum_{i=M+1}^4 50^2$$
We normalize the reward to $[0,1]$ range.
This choice of the reward function is motivated by our early experiments in which we found that random search can be a strong baseline. To highlight the potential of graph based search space we decided to use a reward which is difficult to optimize using a random search.

\begin{wrapfigure}{r}{0.5\textwidth}
\vskip -0.35in
\centering
\includegraphics[width=1.0\linewidth]{figures/nn_addlayer_graph.pdf}
\caption{Graph search space for Cifar10. %experiments. %The controller can terminate at any moment, and conditional decisions are possible within each layer.
}
\label{fig:nn_search_space}
\end{wrapfigure}


% DESCRIPTION OF HOW THE TASK IS REPRESENTED WITH THE SEARCH SPACES
Figure~\ref{fig:branch_vis} illustrates how the ``select an optimizer'' task may be defined as linear and graph search space.
Both search spaces have one state to choose the optimizer, and then four states for each optimizer choice.
The main difference is that the graph search space allows one to build a tree structure having a branch dedicated to each optimizer specific list of hyperparameters.
The linear formulation requires flattening the tree structure into a sequence and choosing the hyperparameters of unused optimizers.



% EXPERIMENT HPARAMS
Again, the reward is normalized to $[0,1]$, and the controller is trained with REINFORCE with learning rate 0.0001 and entropy regularization 0.8.

% RESULTS DISCUSSION
The maximum reward achieved by each time step is shown in Figure~\ref{fig:addlayers_results} for environment with two branches (left) and four branches (right).
Similar to results on the previous toy task, the graph search space improves optimization speed.
We observe a larger benefit in the environment with more branches.


\subsection{Dynamic number of layers}


We experiment on an image classification task. As illustrated by the toy tasks, the key benefit of graph search space lies in the improved convergence speed. In particular, the controller updates only the weights corresponding to the states used to generate the current model.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{figures/graph_exp_cifar10_shaded.pdf}
\caption{Moving average (left) and best (right) reward averaged across 5 replicas for Cifar10. % Graph search space leads to faster convergence, and higher maximum reward.
}
\label{fig:nn_learning_curves}
\end{center}
\end{figure}



% DESCRIPTION OF THE TASK
We experiment on the Cifar10 dataset \citep{cifar-10} and use a similar search space to \citet{tan2018}. The key innovation of~\citet{tan2018} is using a \emph{hierarchical} search space, in which a each of the $7$ layers of the model can be defined individually.
To adapt the search space to Cifar10 we reduce the maximum number of filters, the number of repetitions of each layer, and the number of layers. Finally, we slightly extend the complexity of each layer by allowing the controller to pick the non-linearity and the expansion ratio in squeeze-and-excite layers. %Details are given in the Appendix.
%
% DESCRIPTION OF HOW THE TASK IS REPRESENTED WITH THE SEARCH SPACES
In contrast to the linear search space used in ~\citep{tan2018} we allow the controller to pick the number of layers. We append an extra decision after each final state of the layers whether or not to continue extending the network. The number of layers is capped at $6$. See also Figure ~\ref{fig:nn_search_space} for illustration. 




% EXPERIMENT HPARAMS
%To make the experiment more realistic, we use the state-of-the-art PQT optimizer~\citep{abolafia2018neural}.
Due to the higher resource requirement of this line of experiments we use the more sample efficient Priority Queue Training algorithm~\citep{abolafia2018neural}.
We pick learning rate $0.001$, and the entropy regularization $0.8$.
We sample $1500$ architectures in total. The generated models are trained for $20$ epochs instead of the standard $200$ epochs required to reach state of the art results on Cifar10. 


\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{figures/graph_exp_imagenet.pdf}
\caption{Moving average (right) and best (left) reward for Imagenet. % Graph search space leads to faster convergence, and higher maximum reward.
}
\label{fig:imagenetsearch}
\end{center}
\end{figure}

% NOTE: 14 tells wrapfigure when to stop wrapping
%\begin{wrapfigure}[15]{r}{0.35\textwidth}
%\begin{center}
%\includegraphics[width=1.0\linewidth]{figures/graph_exp_imagenet.pdf}
%\caption{Best reward over time for the ImageNet task.
%%We compare our proposed graph search space with linear search space.
%}
%\label{fig:imagenetsearch}
%\end{center}
%\end{wrapfigure}

Results are summarized in Figure~\ref{fig:nn_learning_curves}. Using the graph search space leads to finding a better architecture, approximately $84\%$ accuracy on Cifar10 compared to $82\%$ of the best model generated using the linear search space.
Note that these results are not meant to reach state-of-the-art performance since the sampled models are trained on a significantly smaller training set and the models are much smaller than state-of-the-art models.
Avoiding training to convergence is the standard methodology for NAS experiments ~\citep{tan2018}. This approach allows to sample a higher number of models. Standard NAS methodology would require to select the best architectures found and train them on the full training set to be able to compare with state-of-the-art results, but this is beyond the scope of this work, that focuses on the analysis of the graph search space.

%See Appendix for details.

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.7\linewidth]{figures/NNexp1.pdf}
% \caption{Maximum (left) and average (right) test accuracy for the Cifar10 task. Graph search space leads to faster convergence, and higher maximum reward.}
% \label{fig:nn_learning_curves}
% \end{center}
% \end{figure}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We have also evaluated the proposed graph search space on ImageNet dataset. Figure \ref{fig:imagenetsearch} shows the best reward obtained graph and linear search space. The graph search experiment converges faster and reaches higher accuracy than linear search space.



==> Graph Nips19/figures/figure_sources.tex <==
fsm_illustration.pdf: https://docs.google.com/drawings/d/1L43wf53zVwNThAKbyz7XwhWiu-kkLteT9GPbDLTyMpk/edit?usp=sharing

architecture.pdf: https://docs.google.com/drawings/d/1teeRiuv3jmgQh3rmXXhouHMIbC4W6qhfmC1YYD9oJ7w/edit?usp=sharing

==> Graph Nips19/introduction.tex <==
\section{Introduction}

%Deep neural networks have yielded success in many supervised learning problems~\citep{DBLP:journals/nature/LeCunBH15}.
%However, 
Neural network design requires many decisions, involving human expertise and time. AutoML speeds up this process by automating some of these decisions~\citep{DBLP:journals/corr/abs-1810-13306}.
%AutoML algorithms may be used to design different aspects of the downstream learning algorithm, from tuning individual hyperparameters, to building architectures, or composing parametric optimization functions.
%AutoML algorithms are usually based on an optimization routine, for which many strategies have been proposed: 
%random search~\citep{Bergstra:2012:RSH:2188385.2188395},
%evolutionary algorithms~\citep{DBLP:journals/corr/abs-1802-01548},
%and Bayesian optimization~\citep{raiders13-workshop,Hutter:2011:SMO:2177360.2177404}.
%
Neural Architecture Search (NAS), as used in ~\citep{zoph2017}, is an approach to AutoML that uses a neural network (``the controller'') to explore different architectures and find the best.
The parameters of the controller's Neural Network are optimized to maximize the performance of generated networks on the downstream task.
This approach has achieved many recent successes \citep{zoph2017b,ramachandran2018searching,bello2017neural} %,wichrowska2017learned}
%, with automatic design of RNN cells~\citep{zoph2017},
%convolutional blocks~\citep{zoph2017b},
%activation functions~\citep{ramachandran2018searching} and
%optimizers~\citep{bello2017neural,wichrowska2017learned}.

% and data augmentation strategies~\citep{cubuk2018autoaugment}.

The success of NAS hinges on the definition of the search space of architectures. %State-of-the-art
Standard search spaces are defined as a linear chain of decisions and a set of available actions for each decision.
For example, the first decision might be ``select the learning rate'' and the corresponding set of actions might be: $\{0.1, 0.01\}$, and the second decision might be ``choose the number of layers'' and its set of available actions might be: $\{1, 2, 3\}$.
%Each possible sequence of actions defines a single architecture.
The controller samples one architecture by sampling one action for each decision. % in the fixed sequence.
However, this formalism hinders the application of NAS to problems that are difficult to define as a linear sequence of actions.
% TODO: give an example.

For example, consider a search space that first picks between more optimizers and then chooses the hyperparameters for the picked optimizer. Performing search over this space using a static sequence forces the controller to make decisions about hyperparameters of all optimizers, rather than only of the picked one. Or as another example, consider a search space that stacks an arbitrary number of convolutional layers and choose different parameters for every added convolution, with a linear search space this iterative component can be represented only by rolling out the loop for a fixed number of iterations.

The main goal of this paper is to lift the limitation of the linear search space for NAS methods. % Inspired by other approaches to AutoML~\citep{raiders13-workshop},
We construct the search spaces as a graph, where each decision is a vertex and each action is an edge.
Thus the sequence of decisions defining an architecture is not fixed but is determined dynamically by the choices of actions.
With this approach the controller may branch and iterate over states.
%, both natural processes in architecture design, resulting in more efficient optimization, as we will show in our experiments.
%
% Furthermore, search spaces including multiple branching and iterative components interacting with each other are not feasibly represented with linear search space.\neil{Make more concrete, or move to Sec 2 and elaborate further there.}
% Graph search spaces enable the modelling of higher complexity search spaces that can generate new classes of architectures.
%
To perform NAS over the proposed graph search space, we design a novel neural controller, capable of dynamically selecting a path through the graph and condition the actions' distributions on the the prior actions.
%The proposed graph search space may replace static linear search spaces used by any neural optimizers, therefore this technology can be used in conjunction with other advances in neural architecture search.


==> Graph Nips19/methods.tex <==
%\section{Neural Architecture Search Over a Graph Search Space}

% SECTION SUMMARY
%In this section we describe the two main contributions of this paper: 1) the generalization of NAS to a graph search space; 2) the dynamic neural architecture controller, capable of learning to search over graph search spaces.

\section{Neural architecture search as a walk in a graph}

% NAS OVERVIEW
NAS aims to find the optimal architecture for a given ML task.
To do this, NAS takes an iterative approach.
At each iteration, a generative neural network, called the \emph{controller}, proposes a new architecture.
Next, this architecture is trained and evaluated on the ML task.
Finally, the evaluation metric is used as a reward to update the controller, using an RL algorithm.

% PRIOR SS FORMALISM FOR NAS
\citet{zoph2017} propose to model the search space as a fixed length sequence of states $s_{1:T}$: one state for each decision.
This approach allows to implement the controller as an RNN.
In each state $s_t$ the controller takes one of the available actions $a_t$. The final sequence of actions $a_{1:T}$ defines the new architecture to be trained and evaluated.

% LIMITATIONS OF PRIOR SS FORMALISM FOR NAS
Modeling the search space as a static length sequence has important limitations. For example, consider a search space that first selects an optimizer and then chooses the hyperparameters for the selected optimizer. Performing search over this space using a static sequence of decision forces the agent to make decisions about hyperparameters of all optimizers, rather than only the selected one.
This is an example of a search space branching.
In general, a linear search space cannot efficiently model either branching or iterative search spaces.

% NOVEL GRAPH SS FORMALISM FOR NAS
To overcome these limitations, we propose to model the search space as a directed graph, 
$\mathcal{G}=(V,A)$,
where each state is represented by a vertex,  $v_{t} \in V$,
and each action is represented by a directed edge, $a_{t} \in A $. % , where $A = V \times V$. % in $A \in V \times V$.
Note that this formalism allows for multiple edges between each pair of vertices, and the graph can be cyclic.
Each path from the start state to a terminal state yields a sequence of actions defining an architecture.

% DETAILS OF HOW THE GRAPH SS ALLOWS TO BUILDS SEQUENCES OF ACTIONS
When traversing the graph, paths are sampled, starting from the start state $v_0$.
Actions are sampled from the distributions learned by the controller $p_{v_t}(a_t)$. The next vertex, $v_{t+1}$, is determined by following the sampled edge $a_t$.
The walk is terminated upon reaching any of the terminal vertices.
After termination, the sampled architecture is defined by the sequence of actions $(a_1,\ldots,a_T)$.
Note that $T$ does not have to be constant, and each state can be visited multiple times. 
% For an example see Figure~\ref{fig:search_space}.

% I think it does't add much, there are many visualizations
% \begin{figure}[t]
% \centering
% \subfigure[Search space represented as a sequence]{\includegraphics[width=0.49\linewidth]{figures/new_fig1a.pdf}}
% \subfigure[Search space represented as a graph]{\includegraphics[width=0.49\linewidth]{figures/fig1b.pdf}}
% \caption{
% Example search space defining two design choices: 
% 1) whether to add a layer, 2) what optimization scheme to use.
% This is configured as a linear search space on the left (a) and as a graph search space on the right (b).
% In the graph instatiation, the controller does not have to make unnecessary decisions: if it chooses not to use Adam, it still has to choose a value for Adam's $\beta_1$.
% Also, the graph search space allows to create a distinct state for choosing the learning rate for each optimizer choice, easing the learning of eventual conditioning.
% \label{fig:search_space}}
% \end{figure}

\section{Dynamic Neural Controller}
\label{sec:arch}

% % \begin{figure}[t]
% \begin{wrapfigure}{r}{0.5\textwidth} 
% \begin{center}
% \includegraphics[width=1.0\linewidth]{figures/architecture.pdf}
% \caption{
% Architecture for one timestep of the dynamic controller.
% \label{fig:architecture}
% }
% \end{center}
% \end{wrapfigure}
% % \end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.7\linewidth]{figures/architecture.pdf}
\caption{
Architecture for one timestep of the dynamic controller. Inputs are highlighted in green, outputs in blue. The timestep-independent network is highlighted in red, the timestep-dependent network in yellow.
\label{fig:architecture}
}
\end{center}
\end{figure}

% CONTROLLER INTRO, HIGHLIGHTS THE NOVELTY: DYNAMIC
To optimize over a graph search space, we propose a modification of the RNN-based neural controller model from~\citet{zoph2017}.
The proposed architecture allows the controller to sample a path from an arbitrary graph, while dynamically setting the sequence of RNN steps to match the sequence of sampled states.
A dynamic architecture is needed to explore graph search spaces, since each action distribution is inferred by a distinct portion of the controller architecture,
and the action distribution to sample from at a given timestep $t$ is determined only after prior timestep $t-1$ is executed.
Instead, for the linear search space, each RNN timestep $t$ always correspond the same action distribution, thus allowing to work with a static controller architecture.

% DETAILS OF THE ARCHITECTURE
Figure~\ref{fig:architecture} depicts the architecture for one timestep of the dynamic RNN controller.
Inputs are highlighted in green, outputs in blue. The timestep-independent network is highlighted in red, the timestep-dependent network in yellow.
At each timestep, the controller takes as input: 1) the current state $v_t$, 2) the previous action $a_{t-1}$, 3) the RNN cell state.
These inputs are aggregated by the timestep independent network.
This is the part of the network whose parameters are the same at each timestep, which includes the action and state embedding tables.
The embeddings of $a_{t-1}$ and $v_t$ are aggregated with a fully connected network. 
Then, this aggregation is the input to an LSTM RNN cell.
%Which has the function of conditioning on learned representation of the prior actions sequence. % carried by the RNN state.
The following portion of the architecture is timestep dependent.
It has the function of inferring the action distribution of the current state $v_t$.
%Note that the shapes and parameters of this part of the architecture can be determined only after $a_{t-1}$ is sampled at the previous timestep.
%Thus it is set dynamically as the actions sequence is sampled.
The outputs are: 1) the action $a_t$ sampled from the timestep dependent action distribution, 2) the next state $v_{t+1}$ determined by $a_t$ 3) the new RNN state.




% TRAINING?
The training is analogous to~\citep{zoph2017}.
The controller learns the action distributions with the objective of maximizing the expected reward of the generated architectures using policy gradient methods.

% DISCUSSION
Notice that the dynamic controller is not required to visit all the states in the search space. This brings multiple benefits that might improve the sample efficiency and stability the controller. Firstly, the controller visits less states, making credit assignment easier. Secondly, gradient updates are performed only for actions that are relevant to the generated model.

%This reduces the variance of the policy gradient updates ~\citep{greensmith2004variance}.





==> Graph Nips19/related_work.tex <==
\section{Related Work}

% I think this is too general for related work in a workshop paper
The complexity of model engineering in machine learning is widely recognized.
Recent successes in automated model design have spurred further work in learning to learn~\citep{thrun2012learning}.
A variety of optimization methods have been proposed to search over architectures, hyperparameters, and learning algorithms.
These include random search \citep{bergstra2012random}, 
parameter modeling \citep{bergstra2013making}, 
meta-learned hyperparameter initialization \citep{feurer2015initializing},
deep-learning based tree searches over a predefined model-specification language \citep{negrinho2017deeparchitect},
learning of gradient descent optimizers \citep{wichrowska2017learned,bello2017neural},
and learning to generate network weights directly~\citep{ha2016hypernetworks,brock2017smash}.
An emerging body of neuro-evolution research has adapted genetic algorithms for these complex optimization problems \citep{conti2017improving}, including to set the parameters of existing deep networks \citep{such2017deep}, 
evolve image classifiers \citep{real2017large},
and evolve generic deep neural networks \citep{miikkulainen2017evolving}.

% RL based approaches
Our work is most closely related to deep RL based methods for auto ML.
Neural Architecture Search (NAS)~\citep{zoph2017} introduced the idea to use deep neural network controller, trained with RL, to generate architecture configurations.
NAS was applied to construct Convolutional Neural Networks (CNNs) for the CIFAR-10 task and Recurrent Neural Networks (RNNs) for the Penn Treebank tasks. 
Significant efforts have been made to achieve increased sample efficiency efficient using a progressive search procedure~\citet{liu2017progressive}, parameter sharing~\citep{cai2017reinforcement,pham2018efficient}, or transfer learning~\citep{wong2018transfer}.

This paper proposes a more expressive formalism for defining model architecture search space for RL based approaches, by generalizing the linear search spaces to graphs.
Extension of linear search spaces to tree structures have been proposed in prior work in the domain of automatic model selection and hyperparamter tuning for approaches based on Bayesian Optimization. These include using specific kernels  ~\citep{raiders13-workshop} or random forests ~\citep{thornton2013auto} to model the acquisition function.

While we focus on RL approaches to NAS, there is a large literature on alternative formulations of NAS. For instance, \citet{pham2018,liu2018darts} proposes to share parameters of all child networks, which allows for drastically faster convergence. However, this was shown to force using a rather limited search space~\citep{sciuto2019evaluating}.

% Other recent publications have also applied RL to automate architecture generation. 
% %These include MetaQNN, a Q-learning algorithm that sequentially chooses CNN layers \citep{baker2016designing}. 
% \citet{baker2016designing,zhong2018practical} use Q-learning to generate entire CNNs or convolutional blocks.
% These works consider one layer selection, including operands, to be a single state.
% In principle, these works can implement a highly flexible search space, however,
% in practice the state space would grow very rapidly if many atomic operations with complex argument structures were added.


% Program synthesis
%\textcolor{red}{a little on program synthesis}

==> acknowledgements.tex <==
\section{Acknowledgements}
We would like to thank
Tomas Effenberger,
David Dohan,
Damien Vincent,
Sylvain Gelly,
Noe Lutz,
Vijay Vasudevan,
Quoc Le and the whole
Google AI team in Zurich for influencing and contributing to the ideas and results presented in this paper.

==> figures/figure_sources.tex <==
fsm_illustration.pdf: https://docs.google.com/drawings/d/1L43wf53zVwNThAKbyz7XwhWiu-kkLteT9GPbDLTyMpk/edit?usp=sharing

architecture.pdf: https://docs.google.com/drawings/d/1teeRiuv3jmgQh3rmXXhouHMIbC4W6qhfmC1YYD9oJ7w/edit?usp=sharing
